Detection and Classification of Bipartite and Multipartite Entangled States

The detection and classification of entanglement properties in a two-qubit and a multi-qubit system is a topic of great interest. This topic has been extensively studied, and as a result, we discovered various approaches for detecting and classifying multi-qubit, in particular three-qubit entangled states. The emphasis of this work is on a formalism of methods for the detection and classification of bipartite as well as multipartite quantum systems. We have used the method of structural physical approximation of partially transposed matrix (SPA-PT) for the detection of entangled states in arbitrary dimensional bipartite quantum systems. Also, we have proposed criteria for the classification of all possible stochastic local operations and classical communication (SLOCC) inequivalent classes of a pure and mixed three-qubit state using the SPA-PT map. To quantify entanglement, we have defined a new measure of entanglement based on the method of SPA-PT, which we named as "structured negativity". We have shown that this measure can be used to quantify entanglement for negative partial transposed entangled states (NPTES). Since the methods for detection, classification and quantification of entanglement, defined in this thesis are based on SPA-PT, they may be realized in an experiment.

==> Abreviation/abrvn.tex <==
\addcontentsline{toc}{chapter}{List of Abbreviations}
\chapter*{List of Abbreviations}
\thispagestyle{empty}
%
%$\begin{array}{cc}
%  CMB & Cosmic Microwave Background \\
%  SNe Ia & Supernova Ia
%\end{array}$

%\noindent\hrulefill


==> Summary/Anu1scope.tex <==
%\thispagestyle{empty}
%\addcontentsline{toc}{chapter}{Summary and future scope of the work}
\chapter{Conclusion and Future Scope}
\section{Conclusion}
\noindent This thesis as a whole may be considered as an extensive review of the detection and classification of arbitrary dimensional bipartite and three-qubit systems, where not only detailed references to the literature have been furnished, but also new and original results have been obtained. We have analyzed the concepts of entanglement detection and classification using methods that may be realized experimentally.\\
In chapter 2, we have explored the methods that exist in the literature and that deal with the detection of entanglement in the bipartite system. Although different criteria are available in the literature for the detection of entanglement, most of them are not physically realizable such as partial transposition (PT) criteria, realignment criteria, range criteria, reduction criteria, etc. Thus, they cannot be implemented in a laboratory. In this chapter, we have proposed three different criteria for the detection of bipartite  NPTES using SPA-PT. Since SPA-PT may be realized in an experiment and thus, the criteria defined in chapter 2 may be realized physically. Moreover, since the closed formula for concurrence is still not known for higher dimensional mixed bipartite systems, so we have derived the lower and upper bound of the concurrence that may be implemented in the laboratory. The first criterion detects NPTES if and only if the average fidelity of two quantum states, which are described by the density matrix $\rho_{AB}$ and SPA-PT of the witness operator $\widetilde{W}$ is less than a quantity $R$. The quantity $R$ depends on (i) the dimension of the composite Hilbert space and (ii) the parameter that makes the SPA-PT of the witness operator positive semi-definite. The second criterion tells us that the given state is NPTES if and only if the minimum eigenvalue of the SPA-PT of the given state is greater or equal to the difference between the concurrence of the given state and the average fidelity between the given state and its SPA-PT. The lower bound of the concurrence is given in terms of the average fidelity of the state  $\rho_{AB}$ and SPA-PT of the witness operator $\widetilde{W}$ while the upper bound is expressed in terms of the average fidelity of the state $\rho_{AB}$ and it's SPA-PT. The third criterion detects a bipartite NPTES $\rho_{AB}$ if and only if $U^{ent}<\frac{1}{2}$ where the quantity $U^{ent}$ depends on the average fidelity of the state $\rho_{AB}$, it's SPA-PT and the concurrence of the state $\rho_{AB}$. The obtained bounds depend on the average fidelity of two quantum states and the average fidelity can be realized in an experiment. Thus, all the entanglement detection criteria obtained in chapter 2, may be realized experimentally. Furthermore, we have defined a way to apply the SPA-PT map on the qutrit-qubit system and explicitly calculated the matrix elements of the density matrix describing the SPA-PT of the qutrit-qubit system. \\
In chapter 3, we considered a pure three-qubit quantum system and studied the problem of classification of a particular type of pure genuine entangled states popularly known as GHZ class of states. It is known that in a three-qubit system, there are two SLOCC inequivalent classes of genuinely entangled states namely GHZ class of states and the W class of states. In general, GHZ class of states can serve as an important class of state for quantum communication purposes. To classify GHZ class into further subclasses, we have defined the classification witness operator for the classification of the canonical form of a pure three-qubit GHZ state. Firstly, we have classified the pure three-qubit GHZ class of states into four subclasses denoted by $S_{1}$, $S_{2}$, $S_{3}$, and $S_{4}$. The motivation for the classification of the pure GHZ class of states into four subclasses is that the GHZ state belonging to $S_{1}$ may be more efficient than the three-qubit GHZ state belonging to $S_{2}$ or $S_{3}$ or $S_{4}$ and vice-versa with respect to some quantum information processing task. For instance, if we consider a GHZ state belonging to subclass $S_{1}$ and a GHZ state belonging to another subclass $S_{2}$ then it can be shown that the tangle of the GHZ state belonging to subclass $S_{1}$ will be greater than the tangle of the GHZ state belonging to subclass $S_{2}$. If any quantum information processing task depends on tangle then the GHZ state belonging to subclass $S_{1}$ will be beneficial in comparison to the GHZ state belonging to $S_2$. On the other hand, we found that the maximal teleportation fidelity of the GHZ states belonging to subclass $S_{2}$ is greater than the GHZ state belonging to subclass $S_{1}$. Therefore, GHZ states belonging to subclass $S_2$ are more suitable shared resource states in teleportation than the GHZ state belonging to subclass $S_1$. Thus, GHZ states belonging to different subclasses have their own importance, and hence if we can detect the subclass of the GHZ state under investigation, then we can use that GHZ state in various quantum information processing tasks accordingly, to get optimal output. Now, in order to identify different subclasses of GHZ class of states, we have constructed different witness operators that can classify the subclasses $S_{i}, i=2,3,4$ from $S_{1}$. Moreover, we have shown that the constructed witness operator can be decomposed into Pauli matrices and hence can be realized experimentally.\\
In chapter 4, we studied the problem of classification of a three-qubit system using $l_1$-norm of coherence. In the literature, the problem of classification of a three-qubit system has been studied using entanglement measures such as tangle and also through the construction of the observables. In a three-qubit system, all the states are classified into six SLOCC inequivalent classes one fully separable state, three biseparable states, and two genuinely entangled states (W class of states and GHZ class of states). While genuine entangled states have entanglement in all the subsystems, biseparable states have entanglement in two of the three subsystems. Biseparable states and genuine entangled states have their own importance and thus, their classification may play a vital role in quantum communication. The classification method based on tangle is not very useful because it cannot discriminate the set of separable states, biseparable states, and W class of states. It happens because the tangle is zero for the set of separable states, biseparable states, and W class of states. In chapter 4, we have used $l_{1}$-norm of coherence to fill this gap for the classification of three-qubit entangled states. Coherence is a basic phenomenon that arises from the superposition principle of quantum mechanics. It can be measured by different measures such as distance measure, relative entropy of coherence, and $l_{p}$-norms. $l_1$-norm is a valid coherence monotone and serves as a useful measure of coherence. In chapter 4, we have calculated the $l_{1}$-norm of coherence of the tensor product of two quantum systems. In order to obtain criteria for the classification of three-qubit states, we have obtained inequalities for biseparable states and separable states in terms of $l_{1}$-norm of coherence. Further, we have shown that if the obtained inequality is violated by any three-qubit state then the state under investigation is neither a biseparable state nor a separable state. Since, for a three-qubit system, we have only three categories of state and if we find that the given state is neither a separable state nor a biseparable state then we can conclude that the state is a genuinely entangled state. At the end of this chapter, we have provided an idea to generalize the obtained results to higher dimensional and multi-qubit systems.\\
In chapter 5, we studied the problem of classification of a three-qubit system using SPA-PT. The methods available in the literature are either incapable of classifying all possible SLOCC inequivalent classes or are not physically realizable. The method defined in chapter 4 for the classification of the three-qubit system is basis dependent and may not be realized physically. To overcome this issue, we have exploited the concept of SPA-PT for the classification of a three-qubit entangled state. Thus in the first part of this chapter, we have taken into account the SPA-PT operation to detect the three-qubit entangled state. To start our study, we have applied partial transposition operation on one of the qubit of the three-qubit system and then studied the entanglement properties of the three-qubit system, which is under investigation. We have defined a way to construct a SPA-PT map for a three-qubit quantum system. With the help of this constructed SPA-PT map, we have provided explicitly the matrix elements of the density matrix describing the SPA-PT of a three-qubit system. We have proposed criteria for the classification of all possible SLOCC inequivalent classes of pure as well as mixed three-qubit states through the SPA-PT map. Thus, the criteria defined in this chapter may classify three-qubit pure and mixed states physically.\\
In chapter 6, we studied the problem of detection and quantification of entangled states in a bipartite quantum system. Measures of entanglement which by definition quantify entangled states may be used for the detection of entanglement. Various entanglement measures exist in the literature such as concurrence, negativity, relative entropy of entanglement, and geometric measure of entanglement that can quantify the amount of entanglement in a two-qubit as well as higher dimensional bipartite pure and mixed state. Out of these, concurrence and negativity are the most popular ones. Although the closed formula for concurrence of mixed two-qubit state can be found in the literature the closed formula does not exist for the concurrence to measure the amount of entanglement in bipartite higher dimensional mixed states. Thus only the lower bound of concurrence is known which helps to estimate the amount of entanglement in the higher dimensional mixed system. On the other hand, negativity is defined for pure as well mixed states in a higher dimensional quantum system. But the problem with negativity is that it is not physically realizable as it depends on the negative eigenvalues of the partially transposed matrix and partial transposition operation corresponds to a non-physical operator. We can overcome this defect by using the structural physical approximation of partial transposition, which by definition transforms a non-physical operator into a physical operator. In this chapter, we have defined a new measure of entanglement using the concept of SPA-PT, which we named "structured negativity". We have shown that it satisfies the properties of a valid entanglement monotone. Since the new measure of entanglement depends on the minimum eigenvalue of the structural physical approximation of the partially transposed matrix, so, it may be realized in an experiment. Moreover, we have obtained a relationship between negativity and structured negativity. Also, we have compared negativity, structured negativity, and the lower bound of the concurrence obtained by Chen et al. \cite{albevario} and found that structured negativity may be a better entanglement measure than negativity and in a few cases, it may perform better than the lower bound of concurrence.
\section{Future Scope}
\noindent %In this section, we will discuss the future scope of this thesis, which is given below:\\
In the literature, various schemes exist for the detection and classification of entangled states in higher dimensional bipartite and multipartite systems but most of them cannot be implemented in the experiment. In the present thesis, we have focussed to overcome this problem and have presented solutions to a few of them, but still, there is a future scope of the thesis, which is discussed below:\\
\textbf{(1)} \textbf{Future scope on the detection of entanglement in higher dimensional bipartite and multipartite quantum system:}\\
\textbf{(1a)} In chapter 1, we studied the problem of detection of entanglement using the SPA-PT method and obtained criteria for the detection of NPTES in an arbitrary dimensional quantum system. In the same way, one may think about the possibility of the development of entanglement detection criteria for PPTES in arbitrary dimensional bipartite systems using SPA-PT.\\
\textbf{(1b)} In chapter 6, we have studied the problem of quantification of bipartite entanglement in arbitrary dimension. To quantify entanglement in an arbitrary dimensional quantum system, we have introduced a new measure of entanglement. The introduced measure is based on SPA-PT and thus the entanglement may be quantified in an experiment. It would be interesting to quantify PPTES using the SPA-PT method.\\
\textbf{(1c)} The construction of an efficient entanglement witness for the detection of entangled states, is very difficult with the increase in the size of the system (dimension and number of qubits). In spite of the difficulty, Zhao et al. \cite{qz} have constructed witness operators for the detection of multipartite GHZ-like states. In the future, it may be possible to develop some method based on the procedure discussed in this thesis for the construction of the efficient witness operator that may detect the class of higher dimensional multipartite W class of states.\\
\textbf{(1d)} In a multipartite system, the detection of Werner states has been studied by constructing a dimension-free entanglement witness using semi-definite programming \cite{fh}. It is important to develop such methods for the detection of entanglement as they can be used for the detection of entanglement in higher dimensional multipartite systems. It opens the door for exploring the problem of detection of entanglement using dimension-free witness operators. One may think of constructing such witnesses for other entangled states that exist in a higher dimensional bipartite and multipartite quantum system.\\
\textbf{(2)} \textbf{Future scope on the classification of entanglement in the three-qubit and multiqubit system:}\\
\textbf{(2a)} In chapter 3, we have considered three-qubit $GHZ$ class of states and divide it into four subclasses $S_1$, $S_2$, $S_3$ and $S_4$. We found that all these four subclasses are important in some quantum information processing tasks. Thus, it is necessary to discriminate them, and hence, we have defined the classification witness operator to classify $S_1$ from $S_i, i=2,3,4$. But still there is a scope to construct classification witness operator that may help to distinguish $S_i$ from $S_j, (i<j, i,j\in\{2,3,4\})$.\\
\textbf{(2b)} In this thesis, we have studied subclasses of three-qubit GHZ class and along the same line of research, one may think of defining different subclasses of the three-qubit W class of states. In this case also, one may investigate whether the subclasses of the W class of states are SLOCC inequivalent or not. It may happen that the states belonging to these subclasses may perform well in quantum communication and thus their classification may also be important. Hence, there is a scope to construct a classification witness operator for the classification of different subclasses of the W class of states.\\
\textbf{(2c)} In chapter 5, we have proposed criteria for the classification of a three-qubit system based on SPA-PT. The obtained criteria are based on the minimum eigenvalue of the maximally entangled three-qubit state. But when we extend these results to a multi-qubit system, the following problem may arise: In $n$-qubit system, where $n>3$, it is very difficult to find maximally entangled states and thus it becomes more difficult to find the minimum eigenvalue of the maximally entangled state to obtain the condition for classification of a three-qubit system using the method of SPA-PT. But in spite of these difficulties, one may obtain the condition for the classification of a four-qubit system because, in a four-qubit system, maximally entangled states are known \cite{gg}.\\
\textbf{(2d)} In chapter 4, we studied the detection and classification of a three-qubit system using  $l_1$-norm of coherence. Our method for the classification of a three-qubit system using $l_1$-norm of coherence is very general and this classification method can be extended to $n$-qubit system, where $n\geq 4$. In the present thesis, we have obtained few results on the classification of the four-qubit system but still, there is a scope to work on it in the future. We have classified separable, biseparable, and genuine three-qubit entangled states but we have not explored the possibility of the classification of two SLOCC inequivalent classes of genuine entangled states, viz, W class and GHZ class. Thus, there is a scope to investigate the classification of GHZ and W class using $l_1$-norm of coherence.\\
\textbf{(2e)} Another problem that arises in a multi-qubit system is that the number of SLOCC inequivalent classes increases with the number of increases in the qubits. Thus, the classification problem becomes more complicated with the increase in the number of qubits. It would be interesting to work on finding the number of different SLOCC inequivalent classes of $n$-qubit system $(n\geq5)$.\\
%Since we have used the SPA-PT method so, it is possible to quantify only negative partial transpose entangled states. Therefore, it opens door to exploring the detection and classification of bound entangled states.\\
%This whole thesis is dedicated to NPTES, in the future, we would like to work on the detection and classification techniques for PPTES such that the methods may be realized experimentally. Also, one may think about the geometrical techniques for the detection and classification of entanglement in the case of PPTES. We would like to work on the applications of entanglement.\\
The field of quantum information theory is definitely worth following over the next decade since everything points toward significant advances. Detection and classification of entanglement are important problems in quantum information theory. To ensure maximum benefit from future surveys, we still need to improve our theoretical understanding of quantum systems, and this thesis is one of many steps toward achieving this.
\begin{center}
	****************
\end{center}



==> Summary/scope.tex <==
%\thispagestyle{empty}
%\addcontentsline{toc}{chapter}{Summary and future scope of the work}
\chapter{Conclusion and Future Scope}
\section{Conclusion}
\indent In the thesis work, we have carried out a study on the accelerating cosmological models of the Universe which has been predicted by many cosmological observations. We have worked on modified theories of gravity to explain it. In chapter 2, the concept of bulk viscosity has been analyzed in $f(R, T)$ gravity to explain the recent accelerated expansion of the Universe. We have observed that the accelerated expansion may be possible for perfect fluid in our model of $f(R, T)$ gravity but the phase transition is not possible. The introduction of bulk viscosity makes the phase transition possible and presents a wide range of possible evolutions of the Universe depending on parameters of the model.\\
\indent Further, chapter 3 deals with the bulk viscosity and matter creation together in $f(R, T)$ gravity. In the literature, both the phenomena have been treated as same cosmological phenomena and some papers treat both as different phenomena. In our study, we have found that although both the phenomena generate effective negative pressure which may explain the accelerated expansion but both have considerably different effects which make both the concepts separate and they exist independently.\\
 \indent It has been shown in chapter 4 that HDE model with Hubble horizon as an IR cut--off may explain the accelerated expansion in $f(R, T)$ gravity without taking interaction between DM and HDE which is not possible in GTR. Further, we have shown that if we consider the viscous HDE then the phase transition may also be achieved. Using statefinder parameters, it has ben found that our model shows the similar behavior as $\Lambda$CDM model and quintessence model for different values of the parameters. Thus, we have observed that $f(R, T)$ gravity has potential to explain the recent accelerated expansion of the Universe. The concept of bulk viscosity presents a mechanism to observe accelerated expansion as well as phase transition of the Universe.\\
\indent In chapter 5, we have studied HDE model in well motivated and established BD theory. We have pointed out that the power--law form of BD scalar field gives a constant as well as time--dependent DP for HDE models in BD theory. It means that the same model describes two types of behavior of the Universe, evolution without phase transition and evolution with phase transition. Therefore, we have proposed a logarithmic form of BD scalar field which is free from this problem. We have shown that HDE model with Hubble horizon as IR cut--off in BD theory with this form of BD scalar field explains early time inflation, medieval time deceleration and late time acceleration of the Universe. This form also plays an important role to avoid cosmic coincidence problem.\\
 \indent We have extended our study to NADE model in chapter 6 and have shown that this model explains the evolution and coincidence problem more effectively with logarithmic form of BD scalar field in comparison of power--law form. Thus, first advantage of this form is that it is free from the constant deceleration parameter problem of power--law, and second is that it explains the evolution of the Universe more effectively and may explain the cosmic coincidence problem.\\
\section{Future Scope}
\indent Our motive is to develop some cosmological models in the framework of modified theories of gravity which may be helpful in order to explain accelerated expansion of the Universe. In this thesis, we have studied $f(R, T)$ gravity because it presents a maximal coupling between matter and geometry which may be useful to explain accelerated expansion of the Universe. The concepts of bulk viscosity, particle creation and HDE have been analyzed in this theory. Further, we have considered BD theory which is a simple extension of GTR to discuss accelerated expansion. We have studied HDE and NADE models in this theory.

\indent As we have mentioned, the $f(R, T)$ theory of gravitation presents a maximal coupling between matter and geometry of the Universe, therefore, it has potential to explain the problems of modern cosmology. Although, a wide range of models have been studied in this theory but still there is a good scope to do work. We have studied only first order Eckart theory of bulk viscosity in $f(R, T)$ gravity, therefore, it may be worthy to discuss the full causal theory of bulk viscosity which may provide better and more general results. The observational cosmology have not been studied considerably in this theory, therefore, there is a lot of scope in this area. The study of structure formation and perturbation theory of $f(R, T)$ gravity are another main fields where a considerable work can be done.\\
\indent We have assumed bulk viscous coefficient as $\zeta=\zeta_0+\zeta_1 H$, however a second order bulk viscous coefficient as $\zeta=\zeta_0+\zeta_1 H+\zeta_2 H^2$ may be considered to describe the late time evolution. In forthcoming paper, we will try to assume such form of $\zeta$ in modified $f(R, T)$ gravity theory. The conservation of energy--momentum tensor is one of the main problem in $f(R, T)$ gravity. Harko has tried to explain the conservation equation through thermodynamics of particle creation. We will try to resolve this problem in future.

\indent The BD theory is an important scalar--tensor theory which provides a natural extension of GTR. We have proposed a logarithmic form of BD scalar field and have shown that HDE model with the logarithmic form of BD scalar field provides some significant results in BD theory. Therefore, it opens door to study the cosmological implications of this form in other aspects of the evolution. It may be interesting to study the behavior of perturbation of BD theory with this form of BD scalar field. It will be worthwhile to analyze whether this form of BD scalar field may provide a mechanism for structure formation to take place. There are many other area like Black hole study, DM problem etc. to discuss in BD theory with this form of BD scalar field. We have considered only Hubble horizon as an IR cut--off to study HDE and NADE models in the framework of BD theory. Therefore, these models may be studied with other IR cut--off candidates like future event horizon, particle event horizon, Grand--Olivers cut--off etc.\\

\noindent\hrulefill


